OPEn: An Open-ended Physics Environment for Learning Without a Task

Humans have mental models that allow them to plan, experiment, and reason in the physical world. How should an intelligent agent go about learning such models? In this paper, we will study if models of the world learned in an open-ended physics environment, without any specific tasks, can be reused for downstream physics reasoning tasks. To this end, we build a benchmark Open-ended Physics ENvironment (OPEn) and also design several tasks to test learning representations in this environment explicitly. This setting reflects the conditions in which real agents (i.e. rolling robots) find themselves, where they may be placed in a new kind of environment and must adapt without any teacher to tell them how this environment works. This setting is challenging because it requires solving an exploration problem in addition to a model building and representation learning problem. We test several existing RL-based exploration methods on this benchmark and find that an agent using unsupervised contrastive learning for representation learning, and impact-driven learning for exploration, achieved the best results. However, all models still fall short in sample efficiency when transferring to the downstream tasks. We expect that OPEn will encourage the development of novel rolling robot agents that can build reusable mental models of the world that facilitate many tasks.

==> dataset.tex <==
\begin{table*}[t]

   % \setlength{\tabcolsep}{3pt}
	\begin{center}
	\begin{tabular}{lccccccc}
	\toprule
         \multirow{2}{*}{Dataset} & \multirow{2}{*}{Interactive} & \multirow{2}{*}{3D scene} & \multirow{2}{*}{Open-ended}
         \multirow{2}{*}{Transfer}
          \midrule  
         Phyre &\times & \checkmark & \times & \times & \times \\
             \midrule 
          IntPhy & \times & \checkmark & \times & \times & \times\\
          \midrule    
        CATER & \times & \checkmark & \times & \times & \times\\
      \midrule    
         CoPhy & \times & \checkmark & \times & \times & \times\\
         \midrule
        CLEVRER & \times & \checkmark & \times & \times & \times\\
         \midrule
         OPHY & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
    \bottomrule
	\end{tabular}
	\end{center}

	\caption{Comparison between OPHY and other physics reasoning benchmarks. OPHY is an open-ended physical enviroment that designed for open-ended learning without a task and model building.}
% 	\data is a video reasoning benchmark created under a fully-controlled environment. The dataset incorporates reasoning tasks from various domains including temporal relation, explanation, prediction and counterfactuals. \data also comes with detailed annotations of object motion, event history and question program for model diagnostics. % \jw{what about making it single-column.}
% 	} % \gc{Move this to supplementary, also include VCR, GQA, Social-IQ}

	\label{tab:dataset_comparison}
\end{table*}
